Structural Parameterization for Graph Deletion Problems over Data Streams

The study of parameterized streaming complexity on graph problems was initiated by Fafianie et al. (MFCS'14) and Chitnis et al. (SODA'15 and SODA'16). Simply put, the main goal is to design streaming algorithms for parameterized problems such that $O\left(f(k)\log^{O(1)}n\right)$ space is enough, where $f$ is an arbitrary computable function depending only on the parameter $k$. However, in the past few years, very few positive results have been established. Most of the graph problems that do have streaming algorithms of the above nature are ones where localized checking is required, like Vertex Cover or Maximum Matching parameterized by the size $k$ of the solution we are seeking. Many important parameterized problems that form the backbone of traditional parameterized complexity are known to require $\Omega(n)$ bits for any streaming algorithm; e.g., Feedback Vertex Set, Even/Odd Cycle Transversal, Triangle Deletion or the more general ${\cal F}$-Subgraph Deletion when parameterized by solution size $k$. Our main conceptual contribution is to overcome the obstacles to efficient parameterized streaming algorithms by utilizing the power of parameterization. To the best of our knowledge, this is the first work in parameterized streaming complexity that considers structural parameters instead of the solution size as a parameter. We focus on the vertex cover size $K$ as the parameter for the parameterized graph deletion problems we consider. At the same time, most of the previous work in parameterized streaming complexity was restricted to the EA (edge arrival) or DEA (dynamic edge arrival) models. In this work, we consider the above mentioned graph deletion problems in the four most well-studied streaming models, i.e., the EA, DEA, VA (vertex arrival) and AL (adjacency list) models.

==> algos.tex <==
\section{The Algorithmic Results}\label{sec:alg}
\noindent
In this Section, we describe the algorithmic results. First, for \cvd parameterized by vertex cover size $K$, we show $(\dea,K^2\log^4 n)$-streamability. By Observation~\ref{obs:vertex_edge_conn}, this implies $(\cM,K^2\log^4 n)$-streamability for all $\cM \in \{\mbox{\ea,\va,\al}\}$. 
 Next, for \fvs, \ect, \Oct and \tdel parameterized by vertex cover size $K$, we show $(\al,K^3)$-streamability. This complements the results in (a) and (b) of Theorems~\ref{theo:lowerbounds} (in Section~\ref{sec:lbproof}) that show that the problems parameterized by vertex cover size $K$ are $(\va,n/p,p)$-hard. Note that by Observation~\ref{obs:vertex_edge_conn}, this also implies that the problems parameterized by vertex cover size $K$ are $(\cM,n/p,p)$-hard when $\cM \in \{\mbox{\ea,\dea}\}$.
\subsection{Algorithm for \cvd in \dea model}
\noindent
Now we give a randomized algorithm for \cvd parameterized by vertex cover size $K$, in the \dea model. The algorithm is inspired by the streaming algorithm for {\sc Vertex Cover}~\cite{ChitnisCEHM15}. Before discussing the algorithm, let us discuss some terms.
\paragraph*{ Pairwise independent hash function} A hash function $h:[n]\rightarrow [m]$ is said to be pairwise independent if for a pair $i,j \in [n]$, $\pr(h(i)=h(j))\leq \frac{1}{m}$. Such a hash function $h$ can be stored efficiently by using $\Oh(\log n )$ bits~\cite{MotwaniR95}. 
%\paragraph*{Dynamic graph stream} In a dynamic graph stream, at each step an edge is either inserted or deleted. So, each input of the stream is either of the form $(e,\mbox{insert})$ or $(e,\mbox{delete})$.
\paragraph*{$\ell_o$-sampler}~\cite{CormodeF14} Given a dynamic graph stream, an $\ell_o$-sampler does the following: with probability at least
$1-\frac{1}{n^c}$, where $c$ is a constant, it produces an edge uniformly at random from the set of edges that have inserted so far but not deleted. If no such edge exists, $\ell_o$-sampler reports {\sc Null}. This means that the $\ell_o$-sampler fails with probability at most $\frac{1}{n^c}$ to return an edge that has been inserted but not deleted. The total space used by the sampler is $\Oh(\log ^3 n)$. 

\begin{theo}
\label{theo:cvd_ub}
\cvd, parameterized by vertex cover size $K$, is $(\dea,K^2\log^4 n)$-streamable.
\end{theo}
\begin{proof}


Let $G$ be the input graph of the streaming algorithm and by assumption $\vc(G) \leq K$. 
Let $h_1,\ldots,h_{\alpha \log n}$ be a set of $\alpha \log n$ pairwise independent hash functions that assigns labels from $[\beta K]$ to $V(G)$, where $\alpha$ and $\beta$ are suitable constants. For each hash function $h_i$ and pair $r,s \in [\beta K]$, let $G_{r,s}^i$ be the subgraph of $G$ induced by the vertex set $\{v \in V(G) : h_i(v) \in \{r,s\}\}$. For the hash function $h_i$ and for each pair $r,s \in [\beta K]$, we initiate an $\ell_o$ sampler for the dynamic stream restricted to the subgraph $G_{r,s}^i$. Therefore, there is a set of $\Oh(K^2)$ $\ell_o$-samplers $\{L^i_{r,s}: r,s \in [\beta K]\}$ corresponding to the hash function $h_i$.

When an edge $(u,v)$ arrives in the stream, that is $(u,v)$ is inserted or deleted, we give the respective input to $L_{h_i(u),h_i(v)}^i$, where $i \in [\alpha \log n]$. At the end of the stream, for each $i \in [\alpha \log n]$, we construct a 
subgraph $H_i$ by taking the outputs of all the $\ell_o$-samplers corresponding to the hash function $h_i$.
Let $H =H_1 \cup \ldots \cup H_{\alpha \log n}$. We run the classical {\sc FPT} algorithm for \cvd on the subgraph $H$ and solution size bound $k$~\cite{saketbook15}, and report \yes to \cvd if and only if we get \yes as answer from the above {\sc FPT} algorithm on $H$. 

In order to prove the correctness of the algorithm we first need a structural result on $G$.
\begin{cl}[(\star)]
\label{clm:cvd_inter}
There exists a partition $\mathcal{P}$ of $V(G)$ into $C_1,\ldots,C_t,I$ such that
 the subgraph induced by each $C_i$, in $G$, is a clique with at least $2$ vertices, and the subgraph induced by $I$ is the empty graph.
\end{cl}
\remove{
\begin{proof}
We start with a partition which may not have the properties of the claim and modify it iteratively such that the final partition does have all the properties of the Claim. Let us start with a partition $\cP$ that does not satisfy the given condition. First, if there exists a part $C_i$ having one vertex $v$, we create a new partition by adding $v$ to $I$. Next, if there exists a part $C_i$ having at least two vertices and the subgraph induced by $C_i$ is not a clique, then we partition $C_i$ into smaller parts such that each smaller part is either a clique having at least two vertices or a singleton vertex\remove{possibly having some neighbors in $C_i$}. We create a new partition by replacing $C_i$ with the smaller cliques of size at least $2$ and adding all the singleton vertices to $I$. Now, let $\cP'$ be the new partition of $V(G)$ obtained after all the above modifications. In $\cP'$, each part except $I$ is a clique of at least two vertices. If the subgraph induced by $I$ has no edges, $\cP'$ satisfies the properties in the Claim and we are done. Otherwise, there exists $u,v \in I$ such that $(u,v) \in E(G)$. In this case, we create a new part with $\{u,v\}$, and remove both $u$ and $v$ from $I$. Note that in the above iterative description, each vertex goes to a new part at most $2$ times - (i) it can move at most once from a part $C_i$ to a smaller part $C_j$ that is a clique on at least $2$ vertices and such a vertex will remain in the same part in all steps afterwards, or it can move at most once from a $C_i$ to $I$, and (ii) a vertex can move at most once from $I$ to become a part of a clique $C_i$ with \comments{at least} $2$ vertices and such a vertex will remain in the same part in all steps after that. Therefore, this process is finite and there is a final partition that we obtain in the end. This final partition has all the properties of the claim.  
\end{proof}}
The correctness of the algorithm follows from the following Claim along with the fact that $H$ is a subgraph of $G$.  
\begin{cl}
\label{lem:cvd_ub_main}
Let $X \subset V(H)$ be such that $H \setminus X$ is a cluster graph. Then $G \setminus X$ is a cluster graph.
\end{cl}
\begin{proof}
Consider a partition $\cP$ of $V(G)$ into $C_1,\ldots,C_t,I$ as mentioned in Claim~\ref{clm:cvd_inter}. Note that our algorithm does not find such a partition. The existence of $\cP$ will be used only for the analysis purpose. Let $\cC=\cup_{i=1}^t C_i$. Note that since $\vc(G) \leq K$, each $C_i$ can have at most $K+1$ vertices, and it must be true that $t\leq \vc(G) \leq K$. In fact we can obtain the following stronger bound that $\vert \cC \vert \leq 2K$: The total number of vertices in $\cC$ is at most $\vc(G) + t$; since $t \leq \vc(G) \leq K$, this gives us the bound of $2K$ on the total number of vertices in $\cC$. %Note that there can be edges between two vertices in same clique, two vertices present in different cliques, or between a vertex in some clique and a vertex in $I$.

Let ${\deg}_G(u)$ denote the degree of $u$ in $G$. A vertex $u \in V(G)$, is said to be of high degree if ${\deg}_G(u) \geq 40K$, and low degree, otherwise. Let $V_h \subseteq V(G)$ be the set of all high degree vertices and $V_{\ell}$ be the set of low degree vertices. Let $E_{\ell}$ be the set of edges having both the end points in $V_{\ell}$. It can be shown that~\cite{ChitnisCEHMMV16,BishnuGKMS18} 
\begin{itemize}
\item[(i)] {\bf Fact-1:} $\size{V_h} \leq K$, $E_{\ell} = \Oh(K^2)$;
\item[(ii)] {\bf Fact-2:} $E_{\ell} \subseteq E(H)$, and ${\deg}_H(u) \geq 4K$ for each $u \in V_h$, with probability $1-\frac{1}{n^{\Oh(1)}}$.
\end{itemize}

Let $\cvdsol(G)  \subset V(G)$ denote a minimum set of vertices such that $G \setminus \cvdsol(G)$ 
is a cluster graph. Now consider the fact that a graph is a cluster graph if and only if it does not have any induced $P_3$. First, we show that the high degree vertices in $G$ surely need to be deleted to make it a cluster graph, i.e., $V_h \subseteq \cvdsol (G)$. Let us consider a vertex $u \in V_h$. 
 As the subgraph induced by $I$ has no edges and $\size{\cC} \leq 2K$, each vertex in $I$ is of degree at most $\size{\cC} \leq 2K$. So, $u$ must be in some $C_i$ in the partition $\mathcal{P}$. As $\deg _G(u) \geq 40K$, using $\vert \cC \vert  \leq 2K$, $u$ must have at least $38K$ many vertices from $I$ as its neighbors in $G$. Thus, there are at least $19K$ edge disjoint induced $P_3$'s that are formed with $u$ and its neighbors in $I$. If $u \notin {\cvdsol}(G)$, then more than $K$ neighbors of $u$ that are in $I$ must be present in $\cvdsol(G)$. It will contradict the fact that $\cvdsol(G) \leq \vc(G) \leq K$. Similarly, we can also argue that $V_h \subseteq \cvdsol(H)=X$ as $\deg _H(u) \geq 4K$ by Fact-2.

Next, we show that the graphs $G \setminus V_h$ and $H \setminus V_h$ are identical. Removal of $V_h$ from $G~(H)$ removes all the induced  $P_3$'s in $G~(H)$ having at least one vertex in $V_h$. Any induced $P_3$ in $G \setminus V_h$ ($H \setminus V_{h}$) must have all of its vertices as low degree vertices. Now, using Fact-2, note that all the edges between low degree vertices are in $H$. In other words, the graph $G \setminus V_h$ and $H \setminus V_h$ are identical. Thus for a set $X \subseteq V(G)$, if $(H \setminus V_h) \setminus X$ is a cluster graph then $(G\setminus V_h) \setminus X$ is also a cluster graph. 
In conclusion, if $X \subseteq V(G)$ is such that $H \setminus X$ is a cluster graph, then $G \setminus X$ is also a cluster graph.
\end{proof}
We are using $\Oh(\log n)$ many hash functions, and each hash function requires a storage of $\Oh(\log n)$ bits.
 There are $\Oh(K^2)$ many $\ell_o$-samplers for each hash function and each $\ell_o$-sampler needs $\Oh(\log^3 n)$ bits of storage. Putting everything together, the total space used by our algorithm is $\Oh(K^2\log^4 n)$.
\end{proof}

\subsection{Algorithms in the \al model}
\noindent
In this Section, we describe a streaming algorithm in the \al model for \fvs, \ect,\Oct and \tdel. First, we define an auxiliary problem \cn and a streaming algorithm for it. This works as a subroutine for our problems.

For a graph $G$ and a parameter $\ell \in \N$, a subgraph $H$ will be called \emph{a common neighbor subgraph} for $G$ if $V(H)=V(G)$ and the edges in $E(H)$ are as follows: (i) $E(H)$ contains the edges of a maximal matching $M$ of $G$ along with the edges whose both the end points are from $V(M)$, (ii) for each pair of vertices $a,b \in V(M)$, the pair has $\min(\size{N_G(a,b) \setminus V(M)},\ell)$ common neighbors in $H$.\remove{(iii) $E(H)$ contains all the edges where .} The parameter $\ell$ will be referred to as the \emph{common neighbor parameter}.

\defproblem{\cn}{A graph $G$ with $\vc(G) \leq K$, parameter $\ell$.}{A common neighbor subgraph of $G$.}

 \cn parameterized by vertex cover size $K$, has the following result.
\begin{lem}
\label{lem:cn}
\cn, parameterized by vertex cover size $K$ and where the common neighbor parameter is $\ell$, is $(\al,K^2\ell)$-streamable. 
\end{lem}
\begin{proof}
We will build a common neighbor subgraph $H$ using the following algorithm. 
We start by initializing $M =\emptyset$ and extend the current maximal matching $M$ of $G$ in the usual way. That is whenever we get an edge $(a,b)$ in the stream, we check whether both $a,b \notin V(M)$. If yes, we replace $M$ by $M \cup \{a,b\}$. Otherwise, we keep $M$ as it is. As $\vc(G) \leq K$, $\size{M} \leq K$.

Recall that we are considering the \al model here. Let $M_u$ be the maximal matching just before we expose the vertex $u$ and $M_u'$ be the maximal matching just after exposing the vertex $u$ and processing the edges adjacent to $u$. Note that by construction these partial matchings $M_u$ and $M'_u$ are also maximal matchings in the subgraph exposed so far.
\begin{cl}
Let $u \in N_G({a,b}) \setminus V(M)$ for some $a,b \in V(M)$. Then $a,b \in V(M_u)$, that is, $u$ is exposed after both $a$ and $b$ are declared as vertices of $V(M)$.  
\end{cl}
\begin{proof}
Observe that if one of $a,b$ is not present in the matching $V(M_u)$, then after $u$ is exposed either $(u,a)$ or $(u,b)$ must be present in $M_u'$. This implies $u \in V(M_u') \subseteq V(M)$, which is a contradiction to $u \in N_G({a,b}) \setminus V(M)$.
\end{proof}
When a vertex $u$ is exposed in the stream, we try to extend the maximal matching $M_u$. Also, we store all the edges  of the form $(u,x)$ such that $x \in V(M_u)$, in a temporary memory $T$. As $\size{M_u} \leq K$, we are storing at most $2K$ many edges in $T$. Now, there are following possibilities.
\begin{itemize}
\item If $u \in V(M_u')$, that is, either $u \in V(M_u)$ or the matching $M_u$ is extended by one of the edges stored in $T$, then we add all the edges stored in $T$ to $E(H)$.
\item Otherwise, for each pair $a, b \in V(M_u)$ such that $a,b \in N_G(u)$, we check whether the number of common neighbors of $a$ and $b$, that are already stored, is less than $ \ell$. If yes, we add both $(u,a)$ and $(u,b)$ to $E(H)$; If no, we do not do anything. Now, we reset $T$ to $\emptyset$.
\end{itemize}  


As $\size{M} \leq K$, $\size{V(M)} \leq 2K$. We are storing at most $\ell$ common neighbors for each pair of vertices in $V(M)$ and the number of edges having both the end points in $M$ is at most $\Oh(K^2)$, the total amount of space used is at most $\Oh(K^2\ell)$.    
\end{proof}

We call the algorithm described in Lemma~\ref{lem:cn}, realizing $(\al,K^2\ell)$-streamability of \cn as $\cA_{cn}$. The following structural Lemma of the common neighbor subgraph of $G$, obtained by algorithm $\cA_{cn}$ is important for the design and analysis of streaming algorithms for \fvs, \ect, \Oct and \tdel. The proof of this structural result is similar to that in~\cite{FOMIN2014468}.

\begin{lem}\label{lem:structure}
Let $G$ be a graph with $\vc(G) \leq K$. Let $H$ be the common neighbor subgraph of $G$ with common neighbor parameter $\const K$, obtained by running the algorithm $\cA_{cn}$. Then the following holds in $H$: For any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$ with $\vert C \vert = \vert C' \vert$ is a subgraph of $H\setminus X$.
\end{lem}

\begin{proof}

Let the common neighbor subgraph $H$, obtained by algorithm $\cA_{cn}$, contain maximal matching $M$ of $G$. First, observe that since $\vc(G) \leq K$, the size of a cycle in $G$ is at most $4K$. 
Now let us consider a subset $X \subseteq V(H)$ such that $\vert X \vert \leq K$. In the reverse direction, suppose $C'$ is a cycle in $H \setminus X$. Then since $H$ is a subgraph of $G$, $C'$ is also a cycle in $G \setminus X$. Therefore, in this direction $C = C'$ and we are done.

In the forward direction, suppose $C$ is a cycle in $G \setminus X$ that is not a cycle in $H \setminus X$. We show that there is a cycle $C'$ of the same length in $H \setminus X$. Let $C = \{u_1,u_2,\ldots,u_t\}$; this ordering on the vertices also gives a natural ordering on the edges $\{e_1,e_2,\ldots,e_s\} \subseteq (E(G) \setminus E(H)) \cap E(C)$. We describe an iterative subroutine that converts the cycle $C$ to $C'$ through a sequence of cycles $C_1,C_2,\ldots C_s$ in $G$ such that $C_s = C'$. In each step $i$, $\vert C_i \vert = \vert C \vert$ and the set of edges in $(E(G) \setminus E(H)) \cap E(C_i)$ is a subset of $\{e_{i+1},e_{i+2},\ldots,e_s\}$. In particular, $C_s = C'$ is a cycle both in $G$ and $H$.

 Suppose we are at step $i$, with $C_i$. For simplicity of notation, we denote the vertex ordering of $C_i$ to be $\{u_1,u_2,\ldots,u_t\}$. We show how we select the cycle $C_{i+1}$. Let $e_{i+1}=(u_j,u_{j+1})$. By definition of the maximal matching $M$ in $G$, exactly one of $\{u_j,u_{j+1}\}$ is in $V(M)$. Without loss of generality, let the vertex in $V(M)$ be $u_j$. Also, if $u_{j+2}$ is the other neighbor of $u_{j+1}$ in $C_i$, then $u_{j+2}$ must also be in $V(M)$ because of maximality of $M$. Now, as $u_{j+1}$ has not been stored as a common neighbor of $u_j,u_{j+2}$ in $H$, the common neighbor subgraph $H$ contains $\const K$ common neighbors. Of these common neighbors, at most $5K$ common neighbors can be vertices in $X \cup C_i$. Thus, there is a vertex $v'$ that is a common neighbor of $u,w$ in $H$ such that $C_{i+1} = \{u_1,u_2,\ldots,u_j,v',u_{j+2},\ldots,u_t\}$ is a cycle that has the same length as $C_i$. Moreover, $(E(G) \setminus E(H)) \cap E(C_{i+1}) \subseteq \{e_{i+2},e_{i+3}\ldots,e_s\}$. 
 If $C_s$ is the final cycle, then by definition of the subroutine $C_s$ is a cycle in $H$ with the same length as $C$. Thus, $C_s$ is the required $C'$ and we are done.

 Hence, for any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$ with $\vert C \vert = \vert C' \vert$ is a subgraph of $H\setminus X$.
 \end{proof}

Now we are ready for our streamability results.
\begin{theo}
\label{theo:cycle_ub}
\fvs, \ect, \Oct and \tdel parameterized by vertex cover size $K$ are $(\al,K^3)$-streamable.
\end{theo}

\begin{proof}
Consider a problem $\Pi$ which is one of the problems \fvs,~\ect,~\Oct, or \tdel.
 Let $(G,k,K)$ be an input for $\Pi$, where $G$ is the input graph, $k$ is the size of the solution of $\Pi$ we are looking for, and the parameter $K$ is such that $\vc(G) \leq K$. Note that for all the above problems, $k \leq K$.
 
 Now, we describe the streaming algorithm for $\Pi$. First, we run the \cn streaming algorithm described in Lemma~\ref{lem:cn} with common neighbor parameter $\const K$, and let the common neighbor subgraph obtained be $H$. We run a traditional FPT algorithm for $\Pi$~\cite{saketbook15} and output \yes if the output on $H$ is YES.
 
 Let us argue the correctness of this algorithm. By Lemma~\ref{lem:structure}, for any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$ with $\vert C \vert = \vert C' \vert$ is a subgraph of $H\setminus X$. In particular, let $X$ be a $k$-sized vertex set of $\Pi$. As mentioned before, $k \leq K$. Lemma~\ref{lem:structure} translates to the following for the different problems:
 \begin{itemize}
  \item If $\Pi$ is \fvs, then the Lemma states that a cycle $C$ is in $G \setminus X$ if and only if there is a cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \ect, then the Lemma states that an even length cycle $C$ is in $G \setminus X$ if and only if there is an even length cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \Oct, then the Lemma states that an odd length cycle $C$ is in $G \setminus X$ if and only if there is an odd length cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \tdel, then the Lemma states that a triangle  $C$ is in $G \setminus X$ if and only if there is a triangle $C'$ in $H \setminus X$.
 \end{itemize}
 Thus, by Lemma~\ref{lem:structure}, $X$ is a solution of $\Pi$ in $H$ if and only if $X$ is a solution of $\Pi$ in $G$. Therefore, we are done with the correctness of the streaming algorithm for $\Pi$.
 
 The streaming complexity of the streaming algorithm for $\Pi$ is same as the streaming complexity for the algorithm $\cA_{cn}$ from Lemma~\ref{lem:cn} with common neighbor parameter $\const K$. Therefore, the streaming complexity is $\Oh(K^3)$.
\end{proof}



==> append.tex <==
\input{problems.tex}
%\input{coro.tex}

\section{Pseudocodes for Section~\ref{sec:cvd} and \ref{sec:minor}}
\label{sec:pseudocode}

\begin{algorithm}[H]
%\scriptsize
\caption{\cvd}
\label{algo_cvd}
\KwIn{A graph $G$ having $n$ vertices in the \dea model,  with  vertex cover size at most $K \in \N$, solution parameter $k \in \N$, such that $k \leq K$.}
\KwOut{A set $X \subset V(G)$ of $k$ vertices such that $G \setminus X$ is a cluster graph if such a set exists. Otherwise, the output is {\sc Null}}
%\LinesNumbered
\Begin
	{
	
	 From a pairwise independent family of hash functions that map $ V(G)$ to $[\beta K]$, choose $h_1,\ldots,h_{\alpha \log n}$ such that each $h_i$ is chosen uniformly and independently at random, where $\alpha$ and $\beta$ are suitable \emph{large} constants. 
	
	For each $i \in [\alpha \log n]$ and $r,s \in [\beta K]$, initiate an $\ell_0$ sampler $L^i_{r,s}$.
	
	\For{ (each $(u,v)$ in the stream)}
	{
	Irrespective of $(u,v)$ being inserted or deleted, give the respective input to the $\ell_0$-samplers $L_{h_i(u),h_i(v)}^i$ for each $i \in [\alpha \log n]$.
	}
	
	For each $i \in [\alpha \log n]$, construct a 
subgraph $H_i$  by taking the outputs of all the $\ell_0$-samplers corresponding to the hash function $h_i$.

Construct $H =H_1 \cup \cdots \cup H_{\alpha \log n}$.

Run the classical {\sc FPT} algorithm for \cvd on the subgraph $H$ and solution size bound $k$~\cite{saketbook15}.

\If{($H$ has a solution $S$ of size at most $k$)}
{Report $S$ as the solution to $G$.}
\Else{
Report {\sc Null}}

}
\end{algorithm}
  \begin{algorithm}[H]
%\scriptsize
\caption{\cn}
\label{algo:cn1}
\KwIn{A graph $G$, with $\vc(G) \leq K$, in the \al model, a degree parameter $d \leq K$, and a common neighbor parameter $\ell$.}
\KwOut{A common neighbor subgraph $H$ of $G$.}
%\LinesNumbered
\Begin
	{
	Initialize $M = \emptyset$ and $V(M)=\emptyset$, where $M$ denotes the current maximal matching.
	
	Initialize a temporary storage $T =\emptyset$.
	
	\For{(each vertex $u \in V(G)$ exposed in the stream)}
	{

			\For{(each $(u,x) \in E(G)$ in the stream)}
			{
				\If{($u \notin V(M) $ and  $x \notin V(M)$)}
				{Add $(u,x)$ to $M$ and both $u,x$ to $V(M)$.}
				 
				 \If{($x \in V(M)$)}
				{ Add $(u,x)$ to $T$.}
			}
			\If{( If $u$ is added to $V(M)$ during the exposure of $u$)}
			{Add all the edges present in $T$ to $E(H)$.}
			\Else
			{ 
				\For{(each $S \subseteq V(M)$ such that $\size{S} \leq d$ and $(u,z) \in T ~\forall z \in S $)}
				{
				\If{($N_H(S)$ is less than $\ell$ )}
				{Add  the edges $(u,z)$ $\forall z \in S$ to $E(H)$.}
				}
			} 
			Reset $T$ to $\emptyset$.
			
	}
	
}
\end{algorithm}



{
\section{Missing Proofs from Section~\ref{sec:cvd}}\label{secappen:cvd}
\label{app:proofcvd}
\begin{proof}[Proof of Claim~\ref{clm:cvd_inter}]
We start with a partition which may not have the properties of the claim and modify it iteratively such that the final partition does have all the properties of the Claim. Let us start with a partition $\cP$ that does not satisfy the given condition. First, if there exists a part $Z_i$ having one vertex $v$, we create a new partition by adding $v$ to $I$. Next, if there exists a part $Z_i$ having at least two vertices and the subgraph induced by $Z_i$ is not a clique, then we partition $Z_i$ into smaller parts such that each smaller part is either a clique having at least two vertices or a singleton vertex\remove{possibly having some neighbors in $C_i$}. We create a new partition by replacing $Z_i$ with the smaller cliques of size at least $2$ and adding all the singleton vertices to $I$. Now, let $\cP'$ be the new partition of $V(G)$ obtained after all the above modifications. In $\cP'$, each part except $I$ is a clique of at least two vertices. If the subgraph induced by $I$ has no edges, $\cP'$ satisfies the properties in the Claim and we are done. Otherwise, there exists $u,v \in I$ such that $(u,v) \in E(G)$. In this case, we create a new part with $\{u,v\}$, and remove both $u$ and $v$ from $I$. Note that in the above iterative description, each vertex goes to a new part at most $2$ times - (i) it can move at most once from a part $Z_i$ to a smaller part $Z_j$ that is a clique on at least $2$ vertices and such a vertex will remain in the same part in all steps afterwards, or it can move at most once from a $Z_i$ to $I$, and (ii) a vertex can move at most once from $I$ to become a part of a clique $Z_i$ with at least $2$ vertices and such a vertex will remain in the same part in all steps after that. Therefore, this process is finite and there is a final partition that we obtain in the end. This final partition has all the properties of the claim.    
\end{proof}

\begin{proof}[Proof of Claim~\ref{lem:cvd_ub_main}]
Consider a partition $\cP$ of $V(G)$ into $Z_1,\ldots,Z_t,I$ as mentioned in Claim~\ref{clm:cvd_inter}. Note that our algorithm does not need to find such a partition. The existence of $\cP$ will be used only for the analysis purpose. Let $\cZ=\cup_{i=1}^t Z_i$. Note that since $\vc(G) \leq K$, each $Z_i$ can have at most $K+1$ vertices, and it must be true that $t\leq \vc(G) \leq K$. In fact, we can obtain the following stronger bound that $\vert \cZ \vert \leq 2K$. The total number of vertices in $\cZ$ is at most $\vc(G) + t$. Since $t \leq \vc(G) \leq K$, the total number of vertices in $\cZ$ is at most $2K$. %Note that there can be edges between two vertices in same clique, two vertices present in different cliques, or between a vertex in some clique and a vertex in $I$.

 A vertex $u \in V(G)$, is said to be of \emph{high degree} if ${\deg}_G(u) \geq 40K$, and \emph{low degree}, otherwise. Let $V_h \subseteq V(G)$ be the set of all high degree vertices and $V_{\ell}$ be the set of low degree vertices in $G$. Let $E_{\ell}$ be the set of edges in $G$  having both the endpoints in $V_{\ell}$. It can be shown~\cite{ChitnisCEHMMV16} that
\begin{itemize}
\item[(i)] {\bf Fact-1:} $\size{V_h} \leq K$, $E_{\ell} = \Oh(K^2)$;
\item[(ii)] {\bf Fact-2:} $E_{\ell} \subseteq E(H)$, and ${\deg}_H(u) \geq 4K$ for each $u \in V_h$, with probability at least $1-\frac{1}{n^{\Oh(1)}}$.
\end{itemize}
Note that Fact-2 makes our algorithmic result for \cvd probabilistic.

Let $\cvdsol(G)  \subset V(G)$ denote a minimum set of vertices such that $G \setminus \cvdsol(G)$ 
is a cluster graph.  Our parametric assumption says that $\size{\cvdsol(G)} \leq \vc(G) \leq K$. Now consider the fact that a graph is a cluster graph if and only if it does not have any induced $P_3$. First, we show that the high degree vertices in $G$ surely need to be deleted to make it a cluster graph, i.e., $V_h \subseteq \cvdsol (G)$. Let us consider a vertex $u \in V_h$. 
 As the subgraph induced by $I$ has no edges and $\size{\cZ} \leq 2K$, each vertex in $I$ is of degree at most $\size{\cZ} \leq 2K$. So, $u$ must be in some $Z_i$ in the partition $\mathcal{P}$. As $\deg _G(u) \geq 40K$, using $\vert \cZ \vert  \leq 2K$, $u$ must have at least $38K$ many vertices from $I$ as its neighbors in $G$. Thus, there are at least $19K$ edge disjoint induced $P_3$'s that are formed with $u$ and its neighbors in $I$. If $u \notin {\cvdsol}(G)$, then more than $K$ neighbors of $u$ that are in $I$ must be present in $\cvdsol(G)$. It will contradict the fact that $\size{\cvdsol(G)} \leq \vc(G) \leq K$. Similarly, we can also argue that $V_h \subseteq \cvdsol(H)=X$ as $\deg _H(u) \geq 4K$ by Fact-2.

Next, we show that an induced $P_3$ is present in $G \setminus V_h$ if and only if it is present in $H \setminus V_h$. Removal of $V_h$ from $G~(\mbox{or}~H)$ removes all the induced  $P_3$'s in $G~(\mbox{or}~H)$ having at least one vertex in $V_h$. Any induced $P_3$ in $G \setminus V_h$ (or $H \setminus V_{h}$) must have all of its vertices as low degree vertices. Now, using Fact-2, note that all the edges, in $G$, between low degree vertices are in $H$. In other words, an induced $P_3$ is present in $G \setminus V_h$ if and only if it is present in $H \setminus V_h$. Thus for a set $X \subseteq V(G)$, if $(H \setminus V_h) \setminus X$ is a cluster graph then $(G\setminus V_h) \setminus X$ is also a cluster graph. 

Putting everything together, if $X \subseteq V(G)$ is such that $H \setminus X$ is a cluster graph, then $G \setminus X$ is also a cluster graph.
\end{proof}

\section{Missing proofs of Section~\ref{sec:minor}}\label{secappen:minor}
\label{app:proofminor}

\begin{proof}[Proof of Lemma~\ref{lem:structure1}]
Let the common neighbor subgraph $H$, obtained by algorithm $\cA_{cn}$, contain a maximal matching $M$ of $G$. First, observe that since $\vc(G) \leq K$, the size of a subgraph $F$ in $G$ is at most $dK$. 
Now let us consider a subset $X \subseteq V(H)$ such that $\vert X \vert \leq K$. First, suppose that $F'$ is a subgraph of $H \setminus X$ and $F'$ is isomorphic to $F$. Then since $H$ is a subgraph of $G$, $F'$ is also a subgraph of $G \setminus X$. Therefore, $F = F'$ and we are done.

Conversely, suppose $F$ is a subgraph of $G \setminus X$ that is not a subgraph in $H \setminus X$. We show that there is a subgraph $F'$ of $H \setminus X$ such that $F'$ is isomorphic to $F$. Consider an arbitrary ordering $\{e_1,e_2,\ldots,e_s\} \subseteq (E(G) \setminus E(H)) \cap E(F)$; note that $s \leq \size{E(F)}$. We describe an iterative subroutine that converts the subgraph $F$ to $F'$ through $s$ steps, or equivalently, through a sequence of isomorphic subgraphs $F_0,F_1,F_2,\ldots F_s$ in $G$ such that $F_0=F$ and $F_s = F'$.

Let us discuss the consequence of such an iterative routine. Just before the starting of step $i \in [s]$, we have the subgraph $F_{i-1}$ such that $ F_{i-1 }$ is isomorphic to $F$ and the set of edges in $(E(G) \setminus E(H)) \cap E(F_{i-1})$ is a subset of $\{e_{i},e_{i+1},\ldots,e_s\}$. In step $i$, we convert the subgraph $F_{i-1}$ into $F_i$ such that $F_{i-1}$ is isomorphic to 
$F_i$. Just after the step $i \in [s]$, we have the subgraph $F_{i}$ such that $F_i$ is isomorphic to $F$ and the set of edges in $(E(G) \setminus E(H)) \cap E(F_i)$ is a subset of $\{e_{i+1},e_{i+2},\ldots,e_s\}$. In particular, in the end $F_s = F'$ is a subgraph both in $G$ and $H$.

Now consider the instance just before step $i$. We show how we select the subgraph $F_{i}$ from $F_{i-1}$. Let $e_{i}=(u,v)$. Note that $e_i \notin E(H)$.  By the definition of the maximal matching $M$ in $G$, it must be the case that $\vert \{u,v\} \cap V(M) \vert \geq 1$. From the construction of the common neighbor subgraph $H$, if both $u$ and $v$ are in $V(M)$, then $e_i=(u,v) \in E(H)$. So, exactly one of $u$ and $v$ is present in $V(M)$. Without loss of generality, let $u \in V(M)$. Observe that $v$ is a common neighbor of  $N_{G}(v)$ in $G$.  Because of the maximality of $M$, each vertex in $N_G(v)$ is present in $V(M)$. Now, as $(u,v) \notin E(H)$, $v$ is not a common neighbor of $N_G(v)$ in $H$. From the construction of the common neighbor subgraph, $H$ contains $(d+2) K$ common neighbors of all the vertices present in $N_G(v)$. Of these common neighbors, at most $(d+1)K$ common neighbors can be vertices in $X \cup F_i$. Thus, there is a vertex $v'$ that is a common neighbor of all the vertices present in $N_G(v)$ in $H$ such that $F_{i+1}$ is a subgraph that is isomorphic to $F_i$. Moreover, $(E(G) \setminus E(H)) \cap E(F_{i+1}) \subseteq \{e_{i+2},e_{i+3}\ldots,e_s\}$. Thus, this leads to the fact that there is a subgraph $F'$ in $H\setminus X$ that is isomorphic to the subgraph $F$ in $G \setminus X$.
 \end{proof}


\begin{proof}[Proof of Theorem~\ref{theo:sub_ub}]
 Let $(G,k,K)$ be an input for \subdel, where $G$ is the input graph, $k \leq K$ is the size of the solution of \subdel, and the parameter $ K$ is at least $\vc(G)$.
 
 Now, we describe the streaming algorithm for \subdel. First, we run the \cn streaming algorithm described in Lemma~\ref{lem:cn1} (and given in Algorithm~\ref{algo:cn1}) with degree parameter $d$ and common neighbor parameter $(d +2) K$, and let the common neighbor subgraph obtained be $H$. We run a traditional FPT algorithm for \subdel~\cite{saketbook15} on $H$ and output \yes if and only if the output on $H$ is YES.
 
 
 Let us argue the correctness of this algorithm. By Lemma~\ref{lem:structure1}, for any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$,  $F \in \cF$ is a subgraph of $G\setminus X$ if and only if  $F'$, such that $F'$ is isomorphic to $F'$, is a subgraph of $H\setminus X$. In particular, let $X$ be a $k$-sized vertex set of $G$. As mentioned before, $k \leq K$.
 Thus, by Lemma~\ref{lem:structure1}, $X$ is a solution of \subdel in $H$ if and only if $X$ is a solution of \subdel in $G$. Therefore, we are done with the correctness of the streaming algorithm for \subdel.
 
 The streaming complexity of \subdel is same as the streaming complexity for the algorithm $\cA_{cn}$ from Lemma~\ref{lem:cn1} with degree parameter $d=\Delta(\cF)$ and common neighbor parameter $(d+2)K$. Therefore, the streaming complexity of \subdel is $\Oh(d \cdot K^{d+1})$.
\end{proof}
 
 
 

\begin{proof}[Proof of Theorem~\ref{theo:minor_ub}]
 Let $(G,k,K)$ be an input for \minordel, where $G$ is the input graph, $k$ is the size of the solution of \minordel we are looking for, and the parameter $K$ is such that $\vc(G) \leq K$. Note that, $k \leq K$.
 
 Now, we describe the streaming algorithm for \minordel. First, we run the \cn streaming algorithm described in Lemma~\ref{lem:cn1} with degree parameter $d$ and common neighbor parameter $(d +2) K$, and let the common neighbor subgraph obtained be $H$. We run a traditional FPT algorithm for \minordel~\cite{saketbook15} and output \yes if and only if the output on $H$ is YES.

 Let us argue the correctness of this algorithm, that is, we prove the following for any $F \in \cF$. 
$G \setminus X$ contains $F$ as a minor if and only if $H \setminus X $ contains $F'$ as a minor such that $F$ and $F'$ are isomorphic, where $X \subseteq V(G)$ is of size at most $K$.  For the only if part, suppose $H \setminus X$ contains $F'$ as a minor. Then since $H$ is a subgraph of $G$, $G \setminus X $ contains $F'$ as a minor. For the 
 if part, let $G \setminus X$ contains $F$ as a minor. By Proposition~\ref{prop:minor-to-sub}, $G \setminus X$ conatins a subgraph $G^{*}$ such that $G^*$ contains $F$ as a minor and $\Delta(G^*) \leq \Delta(F)$. Now, Lemma~\ref{lem:structure1} implies that $H \setminus X$ also contains a subgraph $\hat{G^*}$ that is isomorphic to $G^*$. Hence, $H \setminus X$ contains 
 $F'$ as a monor such that $F'$ is isomorphic to $F$. 

 The streaming complexity of the streaming algorithm for \minordel is same as the streaming complexity for the algorithm $\cA_{cn}$ from Lemma~\ref{lem:cn1} with degree parameter $d=\Delta(\cF)$ and common neighbor parameter $(d+2)K$. Therefore, the streaming complexity for \minordel is $\Oh(d \cdot K^{d+1})$.
\end{proof}}

%\input{lowerboundproofs.tex}

==> coro.tex <==
\noindent
In this Section, we describe a streaming algorithm in the \al model for \fvs, \ect,\Oct and \tdel. First, we define an auxiliary problem \cn and a streaming algorithm for it. This works as a subroutine for our problems.

For a graph $G$ and a parameter $\ell \in \N$, a subgraph $H$ of $G$ will be called \emph{a common neighbor subgraph} for $G$ if 

\begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
\item[(i)] $V(H) \subseteq V(G)$ such that $H$ has no isolated vertex;
\item[(ii)] the edges in $E(H)$ are as follows:
\begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
\item $E(H)$ contains the edges of a maximal matching $M$ of $G$ along with the edges whose both the end points are from $V(M)$, 
\item $E(H)$ contains edges such that for each pair of vertices $a,b \in V(M)$, $\size{N_H(a,b) \setminus V(M)} = \min \{\size{N_G(a,b) \setminus V(M)},\ell\}$.\remove{(iii) $E(H)$ contains all the edges where .}
\end{itemize}
\end{itemize} 
 The parameter $\ell$ will be referred to as the \emph{common neighbor parameter}. Figure~\ref{fig:cngraph} shows an illustration of common neighbor subgraph.
 
 \begin{figure}
  \centering
  \includegraphics[width=1 \linewidth]{cngraph}
  \caption{$(a)$ shows a graph $G$ where $M=\{(v_1,v_2),(v_3,v_4)\}$ is a maximal matching. $(b)$ shows the corresponding common neighbor subgraph $H$ with common neighbor parameter $\ell =2$.}
  \label{fig:cngraph}
\end{figure}
The \cn problem is formally defined as follows.

\defproblem{\cn}{A graph $G$ with $\vc(G) \leq K$, parameter $\ell$.}{A common neighbor subgraph of $G$.}

 \cn parameterized by vertex cover size $K$, has the following result.
 
 \begin{algorithm} 
%\scriptsize
\caption{\cn}
\label{algo_cn}
\KwIn{A graph $G$, with $\vc(G) \leq K$, in the \al model, and a common neighbor parameter $\ell$.}
\KwOut{A common neighbor subgraph $H$ of $G$.}
%\LinesNumbered
\Begin
	{
	Initialize $M = \emptyset$ and $V(M)=\emptyset$, where $M$ denotes the current maximal matching.
	
	Initialize a temporary storage $T =\emptyset$.
	
	\For{(each vertex $u$ exposed in the stream)}
	{

			\For{(each $(u,x)$ in the stream)}
			{
				\If{($u \notin V(M) $ and  $x \notin V(M)$)}
				{Add $(u,x)$ to $M$ and both $u,x$ to $V(M)$.}
				 
				 \If{($x \in V(M)$)}
				{ Add $(u,x)$ to $T$.}
			}
			\If{( If $u$ is added to $V(M)$ during the exposure of $u$)}
			{Add all the edges present in $T$ to $E(H)$.}
			\Else
			{ 
				\For{(each $a,b \in V(M)$ such that $(u,a),(u,b) \in T $)}
				{
				\If{(the number of pairs of edges of the form $(a,x)$ and $(b,x)$ in $E(H)$, is less than $\ell$ )}
				{Add both $(u,a)$ and $(u,b)$ to $E(H)$.}
				}
			} 
			Reset $T$ to $\emptyset$.
			
	}
	
}
\end{algorithm}
\begin{lem}
\label{lem:cn}
\cn, parameterized by vertex cover size $K$ and where the common neighbor parameter is $\ell$, is $(\al,K^2\ell)$-streamable. Moreover the corresponding streaming algorithm is deterministic.
\end{lem}
\begin{proof}
We will build a common neighbor subgraph $H$ using the sketch of the algorithm given in Algorithm~\ref{algo_cn}. 
We start by initializing $M =\emptyset$ and extend the current maximal matching $M$ of $G$ in the usual way. That is whenever we get an edge $(a,b)$ in the stream, we check whether both $a,b \notin V(M)$. If yes, we replace $M$ by $M \cup \{a,b\}$. Otherwise, we keep $M$ as it is. As $\vc(G) \leq K$, $\size{M} \leq K$.

Recall that we are considering the \al model here. Let $M_u$ be the maximal matching just before we expose the vertex $u$ and $M_u'$ be the maximal matching just after exposing the vertex $u$ and processing the edges adjacent to $u$. Note that, by construction these partial matchings $M_u$ and $M'_u$ are also maximal matchings in the subgraph exposed so far. The following Lemma will be useful for the proof.
\begin{cl}
Let $u \in N_G({a,b}) \setminus V(M)$ for some $a,b \in V(M)$. Then $a,b \in V(M_u)$, that is, $u$ is exposed, after both $a$ and $b$ are declared as vertices of $V(M)$.  
\end{cl}
\begin{proof}
Observe that if one of $a,b$ is not present in the matching $V(M_u)$, then after $u$ is exposed, either $(u,a)$ or $(u,b)$ must be present in $M_u'$. This implies $u \in V(M_u') \subseteq V(M)$, which is a contradiction to $u \in N_G({a,b}) \setminus V(M)$.
\end{proof}
When a vertex $u$ is exposed in the stream, we try to extend the maximal matching $M_u$. Also, we store all the edges  of the form $(u,x)$ such that $x \in V(M_u)$, in a temporary memory $T$. As $\size{M_u} \leq K$, we are storing at most $2K$ many edges in $T$. Now, there are the following possibilities.
\begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
\item If $u \in V(M_u')$, that is, either $u \in V(M_u)$ or the matching $M_u$ is extended by one of the edges stored in $T$, then we add all the edges stored in $T$ to $E(H)$.
\item Otherwise, for each pair $a, b \in V(M_u)$ such that $a,b \in N_G(u)$, we check whether the number of common neighbors of $a$ and $b$, that are already stored, is less than $ \ell$. If yes, we add both $(u,a)$ and $(u,b)$ to $E(H)$; else, we do nothing. Now, we reset $T$ to $\emptyset$.
\end{itemize}  


As $\size{M} \leq K$, $\size{V(M)} \leq 2K$. We are storing at most $\ell$ common neighbors for each pair of vertices in $V(M)$ and the number of edges having both the endpoints in $M$ is at most $\Oh(K^2)$, the total amount of space used is at most $\Oh(K^2\ell)$.    
\end{proof}

We call the algorithm described in Algorithm~\ref{algo_cn}, realizing $(\al,K^2\ell)$-streamability of \cn as $\cA_{cn}$. The following structural Lemma of the common neighbor subgraph of $G$, obtained by algorithm $\cA_{cn}$ is important for the design and analysis of streaming algorithms for \fvs, \ect, \Oct and \tdel. The proof of this structural result is similar to that in~\cite{FOMIN2014468}.

\begin{lem}\label{lem:structure}
Let $G$ be a graph with $\vc(G) \leq K$. Let $H$ be the common neighbor subgraph of $G$ with common neighbor parameter $\const K$, obtained by running the algorithm $\cA_{cn}$. Then the following holds in $H$: For any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$ is a subgraph of $H\setminus X$, such that $\vert C \vert = \vert C' \vert$.
\end{lem}

\begin{proof}

Let the common neighbor subgraph $H$, obtained by algorithm $\cA_{cn}$, contains a maximal matching $M$ of $G$. First, observe that since $\vc(G) \leq K$, the size of a cycle in $G$ is at most $4K$. 
Now let us consider a subset $X \subseteq V(H)$ such that $\vert X \vert \leq K$. For the  only if part, suppose $C'$ is a cycle in $H \setminus X$. Then since $H$ is a subgraph of $G$, $C'$ is also a cycle in $G \setminus X$. Therefore, $C = C'$ and we are done.

For the if part, suppose $C$ is a cycle in $G \setminus X$ that is not a cycle in $H \setminus X$. We show that there is a cycle $C'$ of the same length in $H \setminus X$. Let $C = \{u_1,u_2,\ldots,u_t\}$; this ordering on the vertices also gives a natural ordering on the edges $\{e_1,e_2,\ldots,e_s\} \subseteq (E(G) \setminus E(H)) \cap E(C)$; note that $s < t$. We describe an iterative subroutine that converts the cycle $C$ to $C'$ through $s$ steps, or equivalently, through a sequence of cycles $C_0,C_1,C_2,\ldots C_s$ in $G$ such that $C_0=C$ and $C_s = C'$. 

Just before the starting of step $i \in [s]$, we have the cycle $C_{i-1}$ such that $\vert C_{i-1 }\vert = \vert C \vert$ and the set of edges in $(E(G) \setminus E(H)) \cap E(C_{i-1})$ is a subset of $\{e_{i},e_{i+1},\ldots,e_s\}$. In step $i$, we convert the cycle $C_{i-1}$ into $C_i$ such that $\size{C_{i-1}}=\size{C_i}$. Just after the step $i \in [s]$, we have the cycle $C_{i}$ such that $\vert C_i \vert = \vert C \vert$ and the set of edges in $(E(G) \setminus E(H)) \cap E(C_i)$ is a subset of $\{e_{i+1},e_{i+2},\ldots,e_s\}$. In particular, $C_s = C'$ is a cycle both in $G$ and $H$.

 Now consider the instance just before step $i$. For simplicity of notation, we denote the vertex ordering of $C_{i-1}$ to be $\{u_1,u_2,\ldots,u_t\}$. We show how we select the cycle $C_{i}$. Let $e_{i}=(u_j,u_{j+1})$. Note that $e_i \notin E(H)$. By the definition of the maximal matching $M$ in $G$, at least one of $u_j \in V(M)$ or $u_{j+1} \in V(M)$. From the construction of the common neighbor subgraph $H$, if both $u_j$ and $u_{j+1}$ are in $V(M)$, then $e_i=(u_j,u_{j+1}) \in E(H)$. So, exactly one out of $u_j$ and $u_{j+1}$ is present in $V(M)$. Without loss of generality, let $u_j \in V(M)$. Also, if $u_{j+2}$ is the other neighbor of $u_{j+1}$ in $C_{i-1}$, then $u_{j+2}$ must also be in $V(M)$ because of the maximality of $M$. Now, as $(u_j,u_{j+1}) \notin E(H)$, $u_{j+1}$ is not a common neighbor of $u_j$ and $u_{j+2}$ in $H$. From the construction of the common neighbor subgraph, $H$ contains $\const K$ common neighbors of $u_j$ and $u_{j+2}$. Of these common neighbors, at most $5K$ common neighbors can be vertices in $X \cup C_i$. Thus, there is a vertex $v'$ that is a common neighbor of $u_j,u_{j+2}$ in $H$ such that $C_{i+1} = \{u_1,u_2,\ldots,u_j,v',u_{j+2},\ldots,u_t\}$ is a cycle that has the same length as $C_i$. Moreover, $(E(G) \setminus E(H)) \cap E(C_{i+1}) \subseteq \{e_{i+2},e_{i+3}\ldots,e_s\}$. 
 If $C_s$ is the final cycle, then by definition of the subroutine, $C_s$ is a cycle in $H$ with the same length as $C$. Thus, $C_s$ is the required $C'$ and we are done.

 Hence, for any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$ is a subgraph of $H\setminus X$, such that$\vert C \vert = \vert C' \vert$.
 \end{proof}

Now we are ready for our streamability results.
\begin{theo}
\label{theo:cycle_ub}
\fvs, \ect, \Oct and \tdel parameterized by vertex cover size $K$ are $(\al,K^3)$-streamable. Moeover the corresponding streaming algorithms are deterministic.
\end{theo}

\begin{proof}
Consider a problem $\Pi$ which is one of the problems \fvs,~\ect,~\Oct, or \tdel.
 Let $(G,k,K)$ be an input for $\Pi$, where $G$ is the input graph, $k$ is the size of the solution of $\Pi$ we are looking for, and the parameter $K$ is such that $\vc(G) \leq K$. Note that for all the above problems, $k \leq K$.
 
 Now, we describe the streaming algorithm for $\Pi$. First, we run the \cn streaming algorithm described in Lemma~\ref{lem:cn} with common neighbor parameter $\const K$, and let the common neighbor subgraph obtained be $H$. We run a traditional FPT algorithm for $\Pi$~\cite{saketbook15} and output \yes if and only if the output on $H$ is YES.
 
 Let us argue the correctness of this algorithm. By Lemma~\ref{lem:structure}, for any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$, with $\vert C \vert = \vert C' \vert$, is a subgraph of $H\setminus X$. In particular, let $X$ be a $k$-sized vertex set of $\Pi$. As mentioned before, $k \leq K$. Lemma~\ref{lem:structure} translates to the following for the different problems:
 \begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
  \item If $\Pi$ is \fvs, then the Lemma states that a cycle $C$ is in $G \setminus X$ if and only if there is a cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \ect, then the Lemma states that an even length cycle $C$ is in $G \setminus X$ if and only if there is an even length cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \Oct, then the Lemma states that an odd length cycle $C$ is in $G \setminus X$ if and only if there is an odd length cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \tdel, then the Lemma states that a triangle  $C$ is in $G \setminus X$ if and only if there is a triangle $C'$ in $H \setminus X$.
 \end{itemize}
 Thus, by Lemma~\ref{lem:structure}, $X$ is a solution of $\Pi$ in $H$ if and only if $X$ is a solution of $\Pi$ in $G$. Therefore, we are done with the correctness of the streaming algorithm for $\Pi$.
 
 The streaming complexity of the streaming algorithm for $\Pi$ is same as the streaming complexity for the algorithm $\cA_{cn}$ from Lemma~\ref{lem:cn} with common neighbor parameter $\const K$. Therefore, the streaming complexity is $\Oh(K^3)$.
\end{proof}



==> corollary.tex <==
\noindent
In this Section, we describe a streaming algorithm in the \al model for \fvs, \ect,\Oct and \tdel. First, we define an auxiliary problem \cn and a streaming algorithm for it. This works as a subroutine for our problems.

For a graph $G$ and a parameter $\ell \in \N$, a subgraph $H$ of $G$ will be called \emph{a common neighbor subgraph} for $G$ if 

\begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
\item[(i)] $V(H) \subseteq V(G)$ such that $H$ has no isolated vertex;
\item[(ii)] the edges in $E(H)$ are as follows:
\begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
\item $E(H)$ contains the edges of a maximal matching $M$ of $G$ along with the edges whose both the end points are from $V(M)$, 
\item $E(H)$ contains edges such that for each pair of vertices $a,b \in V(M)$, $\size{N_H(a,b) \setminus V(M)} = \min \{\size{N_G(a,b) \setminus V(M)},\ell\}$.\remove{(iii) $E(H)$ contains all the edges where .}
\end{itemize}
\end{itemize} 
 The parameter $\ell$ will be referred to as the \emph{common neighbor parameter}. Figure~\ref{fig:cngraph} shows an illustration of common neighbor subgraph.
 
 \begin{figure}
  \centering
  \includegraphics[width=1 \linewidth]{cngraph}
  \caption{$(a)$ shows a graph $G$ where $M=\{(v_1,v_2),(v_3,v_4)\}$ is a maximal matching. $(b)$ shows the corresponding common neighbor subgraph $H$ with common neighbor parameter $\ell =2$.}
  \label{fig:cngraph}
\end{figure}
The \cn problem is formally defined as follows.

\defproblem{\cn}{A graph $G$ with $\vc(G) \leq K$, parameter $\ell$.}{A common neighbor subgraph of $G$.}

 \cn parameterized by vertex cover size $K$, has the following result.
 
 \begin{algorithm} 
%\scriptsize
\caption{\cn}
\label{algo_cn}
\KwIn{A graph $G$, with $\vc(G) \leq K$, in the \al model, and a common neighbor parameter $\ell$.}
\KwOut{A common neighbor subgraph $H$ of $G$.}
%\LinesNumbered
\Begin
	{
	Initialize $M = \emptyset$ and $V(M)=\emptyset$, where $M$ denotes the current maximal matching.
	
	Initialize a temporary storage $T =\emptyset$.
	
	\For{(each vertex $u$ exposed in the stream)}
	{

			\For{(each $(u,x)$ in the stream)}
			{
				\If{($u \notin V(M) $ and  $x \notin V(M)$)}
				{Add $(u,x)$ to $M$ and both $u,x$ to $V(M)$.}
				 
				 \If{($x \in V(M)$)}
				{ Add $(u,x)$ to $T$.}
			}
			\If{( If $u$ is added to $V(M)$ during the exposure of $u$)}
			{Add all the edges present in $T$ to $E(H)$.}
			\Else
			{ 
				\For{(each $a,b \in V(M)$ such that $(u,a),(u,b) \in T $)}
				{
				\If{(the number of pairs of edges of the form $(a,x)$ and $(b,x)$ in $E(H)$, is less than $\ell$ )}
				{Add both $(u,a)$ and $(u,b)$ to $E(H)$.}
				}
			} 
			Reset $T$ to $\emptyset$.
			
	}
	
}
\end{algorithm}
\begin{lem}
\label{lem:cn}
\cn, parameterized by vertex cover size $K$ and where the common neighbor parameter is $\ell$, is $(\al,K^2\ell)$-streamable. Moreover the corresponding streaming algorithm is deterministic.
\end{lem}
\begin{proof}
We will build a common neighbor subgraph $H$ using the sketch of the algorithm given in Algorithm~\ref{algo_cn}. 
We start by initializing $M =\emptyset$ and extend the current maximal matching $M$ of $G$ in the usual way. That is whenever we get an edge $(a,b)$ in the stream, we check whether both $a,b \notin V(M)$. If yes, we replace $M$ by $M \cup \{a,b\}$. Otherwise, we keep $M$ as it is. As $\vc(G) \leq K$, $\size{M} \leq K$.

Recall that we are considering the \al model here. Let $M_u$ be the maximal matching just before we expose the vertex $u$ and $M_u'$ be the maximal matching just after exposing the vertex $u$ and processing the edges adjacent to $u$. Note that, by construction these partial matchings $M_u$ and $M'_u$ are also maximal matchings in the subgraph exposed so far. The following Lemma will be useful for the proof.
\begin{cl}
Let $u \in N_G({a,b}) \setminus V(M)$ for some $a,b \in V(M)$. Then $a,b \in V(M_u)$, that is, $u$ is exposed, after both $a$ and $b$ are declared as vertices of $V(M)$.  
\end{cl}
\begin{proof}
Observe that if one of $a,b$ is not present in the matching $V(M_u)$, then after $u$ is exposed, either $(u,a)$ or $(u,b)$ must be present in $M_u'$. This implies $u \in V(M_u') \subseteq V(M)$, which is a contradiction to $u \in N_G({a,b}) \setminus V(M)$.
\end{proof}
When a vertex $u$ is exposed in the stream, we try to extend the maximal matching $M_u$. Also, we store all the edges  of the form $(u,x)$ such that $x \in V(M_u)$, in a temporary memory $T$. As $\size{M_u} \leq K$, we are storing at most $2K$ many edges in $T$. Now, there are the following possibilities.
\begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
\item If $u \in V(M_u')$, that is, either $u \in V(M_u)$ or the matching $M_u$ is extended by one of the edges stored in $T$, then we add all the edges stored in $T$ to $E(H)$.
\item Otherwise, for each pair $a, b \in V(M_u)$ such that $a,b \in N_G(u)$, we check whether the number of common neighbors of $a$ and $b$, that are already stored, is less than $ \ell$. If yes, we add both $(u,a)$ and $(u,b)$ to $E(H)$; else, we do nothing. Now, we reset $T$ to $\emptyset$.
\end{itemize}  


As $\size{M} \leq K$, $\size{V(M)} \leq 2K$. We are storing at most $\ell$ common neighbors for each pair of vertices in $V(M)$ and the number of edges having both the endpoints in $M$ is at most $\Oh(K^2)$, the total amount of space used is at most $\Oh(K^2\ell)$.    
\end{proof}

We call the algorithm described in Algorithm~\ref{algo_cn}, realizing $(\al,K^2\ell)$-streamability of \cn as $\cA_{cn}$. The following structural Lemma of the common neighbor subgraph of $G$, obtained by algorithm $\cA_{cn}$ is important for the design and analysis of streaming algorithms for \fvs, \ect, \Oct and \tdel. The proof of this structural result is similar to that in~\cite{FOMIN2014468}.

\begin{lem}\label{lem:structure}
Let $G$ be a graph with $\vc(G) \leq K$. Let $H$ be the common neighbor subgraph of $G$ with common neighbor parameter $\const K$, obtained by running the algorithm $\cA_{cn}$. Then the following holds in $H$: For any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$ is a subgraph of $H\setminus X$, such that $\vert C \vert = \vert C' \vert$.
\end{lem}

\begin{proof}

Let the common neighbor subgraph $H$, obtained by algorithm $\cA_{cn}$, contains a maximal matching $M$ of $G$. First, observe that since $\vc(G) \leq K$, the size of a cycle in $G$ is at most $4K$. 
Now let us consider a subset $X \subseteq V(H)$ such that $\vert X \vert \leq K$. For the  only if part, suppose $C'$ is a cycle in $H \setminus X$. Then since $H$ is a subgraph of $G$, $C'$ is also a cycle in $G \setminus X$. Therefore, $C = C'$ and we are done.

For the if part, suppose $C$ is a cycle in $G \setminus X$ that is not a cycle in $H \setminus X$. We show that there is a cycle $C'$ of the same length in $H \setminus X$. Let $C = \{u_1,u_2,\ldots,u_t\}$; this ordering on the vertices also gives a natural ordering on the edges $\{e_1,e_2,\ldots,e_s\} \subseteq (E(G) \setminus E(H)) \cap E(C)$; note that $s < t$. We describe an iterative subroutine that converts the cycle $C$ to $C'$ through $s$ steps, or equivalently, through a sequence of cycles $C_0,C_1,C_2,\ldots C_s$ in $G$ such that $C_0=C$ and $C_s = C'$. 

Just before the starting of step $i \in [s]$, we have the cycle $C_{i-1}$ such that $\vert C_{i-1 }\vert = \vert C \vert$ and the set of edges in $(E(G) \setminus E(H)) \cap E(C_{i-1})$ is a subset of $\{e_{i},e_{i+1},\ldots,e_s\}$. In step $i$, we convert the cycle $C_{i-1}$ into $C_i$ such that $\size{C_{i-1}}=\size{C_i}$. Just after the step $i \in [s]$, we have the cycle $C_{i}$ such that $\vert C_i \vert = \vert C \vert$ and the set of edges in $(E(G) \setminus E(H)) \cap E(C_i)$ is a subset of $\{e_{i+1},e_{i+2},\ldots,e_s\}$. In particular, $C_s = C'$ is a cycle both in $G$ and $H$.

 Now consider the instance just before step $i$. For simplicity of notation, we denote the vertex ordering of $C_{i-1}$ to be $\{u_1,u_2,\ldots,u_t\}$. We show how we select the cycle $C_{i}$. Let $e_{i}=(u_j,u_{j+1})$. Note that $e_i \notin E(H)$. By the definition of the maximal matching $M$ in $G$, at least one of $u_j \in V(M)$ or $u_{j+1} \in V(M)$. From the construction of the common neighbor subgraph $H$, if both $u_j$ and $u_{j+1}$ are in $V(M)$, then $e_i=(u_j,u_{j+1}) \in E(H)$. So, exactly one out of $u_j$ and $u_{j+1}$ is present in $V(M)$. Without loss of generality, let $u_j \in V(M)$. Also, if $u_{j+2}$ is the other neighbor of $u_{j+1}$ in $C_{i-1}$, then $u_{j+2}$ must also be in $V(M)$ because of the maximality of $M$. Now, as $(u_j,u_{j+1}) \notin E(H)$, $u_{j+1}$ is not a common neighbor of $u_j$ and $u_{j+2}$ in $H$. From the construction of the common neighbor subgraph, $H$ contains $\const K$ common neighbors of $u_j$ and $u_{j+2}$. Of these common neighbors, at most $5K$ common neighbors can be vertices in $X \cup C_i$. Thus, there is a vertex $v'$ that is a common neighbor of $u_j,u_{j+2}$ in $H$ such that $C_{i+1} = \{u_1,u_2,\ldots,u_j,v',u_{j+2},\ldots,u_t\}$ is a cycle that has the same length as $C_i$. Moreover, $(E(G) \setminus E(H)) \cap E(C_{i+1}) \subseteq \{e_{i+2},e_{i+3}\ldots,e_s\}$. 
 If $C_s$ is the final cycle, then by definition of the subroutine, $C_s$ is a cycle in $H$ with the same length as $C$. Thus, $C_s$ is the required $C'$ and we are done.

 Hence, for any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$ is a subgraph of $H\setminus X$, such that$\vert C \vert = \vert C' \vert$.
 \end{proof}

Now we are ready for our streamability results.
\begin{theo}
\label{theo:cycle_ub}
\fvs, \ect, \Oct and \tdel parameterized by vertex cover size $K$ are $(\al,K^3)$-streamable. Moeover the corresponding streaming algorithms are deterministic.
\end{theo}

\begin{proof}
Consider a problem $\Pi$ which is one of the problems \fvs,~\ect,~\Oct, or \tdel.
 Let $(G,k,K)$ be an input for $\Pi$, where $G$ is the input graph, $k$ is the size of the solution of $\Pi$ we are looking for, and the parameter $K$ is such that $\vc(G) \leq K$. Note that for all the above problems, $k \leq K$.
 
 Now, we describe the streaming algorithm for $\Pi$. First, we run the \cn streaming algorithm described in Lemma~\ref{lem:cn} with common neighbor parameter $\const K$, and let the common neighbor subgraph obtained be $H$. We run a traditional FPT algorithm for $\Pi$~\cite{saketbook15} and output \yes if and only if the output on $H$ is YES.
 
 Let us argue the correctness of this algorithm. By Lemma~\ref{lem:structure}, for any subset $X \subseteq V(H)$, where $\vert X \vert \leq K$, a cycle $C$ is a subgraph of $G\setminus X$ if and only if a cycle $C'$, with $\vert C \vert = \vert C' \vert$, is a subgraph of $H\setminus X$. In particular, let $X$ be a $k$-sized vertex set of $\Pi$. As mentioned before, $k \leq K$. Lemma~\ref{lem:structure} translates to the following for the different problems:
 \begin{itemize}[noitemsep,wide=0pt, leftmargin=\dimexpr\labelwidth + 2\labelsep\relax]
  \item If $\Pi$ is \fvs, then the Lemma states that a cycle $C$ is in $G \setminus X$ if and only if there is a cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \ect, then the Lemma states that an even length cycle $C$ is in $G \setminus X$ if and only if there is an even length cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \Oct, then the Lemma states that an odd length cycle $C$ is in $G \setminus X$ if and only if there is an odd length cycle $C'$ in $H \setminus X$.
  \item If $\Pi$ is \tdel, then the Lemma states that a triangle  $C$ is in $G \setminus X$ if and only if there is a triangle $C'$ in $H \setminus X$.
 \end{itemize}
 Thus, by Lemma~\ref{lem:structure}, $X$ is a solution of $\Pi$ in $H$ if and only if $X$ is a solution of $\Pi$ in $G$. Therefore, we are done with the correctness of the streaming algorithm for $\Pi$.
 
 The streaming complexity of the streaming algorithm for $\Pi$ is same as the streaming complexity for the algorithm $\cA_{cn}$ from Lemma~\ref{lem:cn} with common neighbor parameter $\const K$. Therefore, the streaming complexity is $\Oh(K^3)$.
\end{proof}



==> lowerbound-main.tex <==
\vspace{-0.5cm}
\section{$\Omega(n \log n)$ lower bound for \fvs in the \al model}\label{sec:fvs lower bound}
In this Section, we show the following Theorem by reducing from a communication complexity problem \perm~\cite{SunW15}, whose \emph{one way communication complexity} is $\Omega(n \log n)$. The detailed exposition of communication complexity and lower bound results are presented in 
Appendix~\ref{sec:lbproof}. In \perm, Alice gets a permutation $\pi : [n]\rightarrow [n]$ and Bob gets an index $j \in [n \log n]$. The objective of Bob is to decide the value of  $\permxy$, defined as the $j$-{th} bit in the string of $0$'s and $1$'s obtained by concatenating the bit expansions of $\pi(1)\ldots \pi(n)$. In other words, let $\Phi:[n \log n] \rightarrow [n] \times [\log n]$ be a bijective function defined as 
$\Phi(j)=\left( \lceil \frac{j}{\log n} \rceil, j + \log n -\lceil \frac{j}{\log n} \rceil \times \log n  \right)$. For a permutation $\pi: [n] \rightarrow [n]$, Bob needs to determine the value of the $\gamma$-th bit of $\pi \left( \lceil \frac{j}{\log n} \rceil \right)$, where $\gamma={ \left(j + \log n -\lceil \frac{j}{\log n} \rceil \times \log n  \right)}$.

\begin{theo}\label{theo:fvslb}
\fvs is $(\al, n \log n)$-hard.
\end{theo} 
\begin{proof}
\begin{figure}[h!]
  \centering
  \includegraphics[width=0.5 \linewidth]{fvs1}
  \caption{Illustration of Proof of Theorem~\ref{theo:fvslb}. Consider $n=4$. Let $\pi:[4]\rightarrow [4]$ such that $\pi(1)=3, \pi(2)=4, \pi(3)=2$ and $\pi(4)=1$. So the concatenated bit string is $11001001^{{3}}$. In (a), $j=5$, $\Phi(j)=(\psi,\gamma)=(3,1)$, $\permxy=1$, and $G$ contains a cycle. In (b), $j=4$, $\Phi(j)=(\psi,\gamma)=(2,2)$, $\permxy=0$, and $G$ does not contain a cycle.}
  \label{fig:ffvs1}
\end{figure}
\footnotetext{Recall that we take $n$ as a power of $2$. For $1 \leq i \leq n-1$, the bit expansion of $i$ is the usual bit notation of $i$ using $\log_2 n$ bits; the bit expansion of $n$ is $\log_2 n$ many consecutive zeros. For example: Take $n=32$. The bit expansion of $32$ is $100000$. We ignore the bit $1$ and say that the bit expansion of $32$ is $00000$.}
We give a reduction from \perm to \fvs in the \al model when the solution size parameter $k=0$.  The idea is to build a graph $G$ (with $\Delta_{av}(G) =\Oh(1)$) and construct edges according to the input of \perm, such that the output of \perm is $0$ if and only if $G$ is cycle-free.

Let $\cA$ be a one pass streaming algorithm that solves \fvs in \al model using $o(n \log n)$ space. \remove{Now we give a protocol that solves \perm using $o(n \log n)$ space. }Let $G$ be a graph with $4n+2$ vertices $u_1,\ldots,u_n,$ $v_1,\ldots,v_n, u'_1, \dots,$ $u'_n, v'_1,\dots, v'_n, w,$ $w'$. Let $\pi$ be the input of Alice for \perm. See Figure~\ref{fig:ffvs1} for an illustration.

{\bf Alice's input to $\cA$:} Alice inputs the graph $G$ first by exposing the vertices $u_1,\ldots,u_n, v_1,\ldots,$ $v_n$, sequentially. 
(i) While exposing the vertex $u_i$, Alice gives as input to $\cA$ the edges $(u_i,u'_i),(u_i, v_{\pi(i)})$; 
(ii) while exposing the vertex $v_i$, Alice gives the edges $(v_i,v'_i),(v_i,$ $ u_{\pi^{-1}(i)})$ to the input stream of $\cA$.

After the exposure of $u_1,\ldots,u_n, v_1,\ldots,$ $v_n$ as per the \al model, Alice sends the current memory state of $\cA$, i.e the sketch generated by $\cA$, to Bob. Let $j \in [n \log n]$ be the input of Bob and let $(\psi,\gamma) =\Phi(j)$.

{\bf Bob's input to $\cA$:}
 Bob exposes the vertices $u'_1 \dots, u'_n, v'_1,$ $\ldots,$ $ v'_n,w,w'$, sequentially. 
 (i) While exposing a vertex $u'_i$ where $i \neq \psi$, Bob gives the edge $(u'_i,u_i)$ to the input stream of $\cA$; 
 (ii) while exposing $u'_\psi$, Bob gives the edges $(u'_\psi,u_\psi)$ and $(u'_\psi,w')$;  
 (iii) while exposing a vertex $v'_i$, Bob gives the edge $(v'_i,v_i)$, and the edge $(v'_i,w)$ if and only if $\bit(i,\gamma)=1$;
 (iv) while exposing $w$, Bob gives the edge $(w,w')$, and the edge $(w,v'_i)$ if and only if $\bit(i,\gamma)=1$; 
 (v) while exposing $w'$, Bob gives the edges $(w',w)$ and $(w',u'_{\psi})$. 

 Observe that $\Delta_{av}(G)=\Oh(1)$. Now we show that the output of \fvs{} is \no if and only if $\permxy=1$. Recall that $k=0$.

%Also, a cycle in $G$ contains the edges $(u_{p},v_{\pi(p)})$ and , if it exists.  

From the construction, observe that $(w,w'), (w',u'_\psi), (u'_\psi,u_\psi),$ $(u_\psi, v_{\pi(\psi)}), (v_{\pi(\psi)}, v'_{\pi(\psi)}) \in E(G)$.
 When $\permxy =1$, the edge $(v'_{\pi(\psi)},w)$ is present in $G$. 
 So, $G$ contains the cycle $\cC (w,w',u'_{\psi},$ $u_\psi,v_{\pi(\psi)},v'_{\pi(\psi)} )$, that is, the output of \fvs is NO.
 
 On the other hand, if the output of \fvs is NO, then there is a cycle in $G$. From the construction, the cycle is 
 $\cC(w,w',u'_{\psi},u_\psi,v_{\pi(\psi)},v'_{\pi(\psi)})$. As $(v'_{\pi(\psi)},w)$ is an edge, the $\gamma$-{{th}} bit of $\pi(\psi)$ is $1$, that is $\permxy =1$. As the one-way commmunication complexity of \perm is $\Omega(n \log n)$, we obtain that {\sc Feedback Vertex Set} is $(\al, n \log n)$-hard even if $\Delta_{av}(G)=\Oh(1)$ and when $k=0$.
 
  We make the reduction work for any $k$, by adding $k$  vertex disjoint cycles of length $4$ to $G$.
  \end{proof}

\vspace{-0.5cm}
